SALSA VERDE: a machine learning attack on Learning With Errors with sparse small secrets

Learning with Errors (LWE) is a hard math problem used in post-quantum cryptography. Homomorphic Encryption (HE) schemes rely on the hardness of the LWE problem for their security, and two LWE-based cryptosystems were recently standardized by NIST for digital signatures and key exchange (KEM). Thus, it is critical to continue assessing the security of LWE and specific parameter choices. For example, HE uses secrets with small entries, and the HE community has considered standardizing small sparse secrets to improve efficiency and functionality. However, prior work, SALSA and PICANTE, showed that ML attacks can recover sparse binary secrets. Building on these, we propose VERDE, an improved ML attack that can recover sparse binary, ternary, and narrow Gaussian secrets. Using improved preprocessing and secret recovery techniques, VERDE can attack LWE with larger dimensions ($n=512$) and smaller moduli ($\log_2 q=12$ for $n=256$), using less time and power. We propose novel architectures for scaling. Finally, we develop a theory that explains the success of ML LWE attacks.

==> Makefile <==
LATEX=latex
BIBTEX=bibtex
BIBFILE=references.bib
PAPER=picante

TEXFILES = picante.tex \
	intro.tex \
	back.tex \
	method.tex \
	attack.tex \
	results.tex \
	discussion.tex \

EPSFIGS = \

EPSGRAPHS = $(wildcard figures/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) (PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

#$(PAPER).pdf: $(PAPER).dvi
#	dvipdf $(PAPER).dvi

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out


==> figs/transformer_pic.tex <==

\definecolor{DarkGray}{HTML}{68904d}
\definecolor{Orange}{HTML}{ffae42}
%\begin{figure}[h!]
\begin{minipage}[t]{0.45\textwidth}
\small
\centering
\begin{tikzpicture}[
    box/.style={rectangle,draw,fill=DarkGray!20,node distance=1cm,text width=8em,text centered,rounded corners,minimum height=1.5em,thick},
    box2/.style={rectangle,draw,fill=DarkGray!20,node distance=1cm,text width=1em,text centered,rounded corners,minimum height=0.5em,thick},
    arrow/.style={draw,-latex',thick},
  ]
  \node [box] (ffne) {FCNN};
  
  
  \node [box2,above=0.5 of ffne] (tok2) {c$_2$};
  \node [box2,left=0.25 of tok2] (tok1) {c$_1$};
  \node [box2,right=0.25 of tok2] (tok3) {c$_3$};
  \node [above=0.2 of tok2]{Encoder output};
  \node [box,below=0.23 of ffne,fill=Orange] (selfatt){Self-attention};  
  \node [label={[rotate=90]160:Layer 1},rectangle,draw,dashed,inner sep=0.7em,fit=(selfatt) (ffne)] (encoder1) {};

  \node [box2,below=0.4 of selfatt] (se){x$_2$};
  \node [box2,left=0.25 of se] (se2){x$_1$};
  \node [box2,right=0.25 of se] (se3){x$_3$};
  \node [box,below=0.23 of se] (embed) {Embedding};
  \node [below=0.3 of embed] (inp2) {\texttt{2}};
\node [right=0.25 of inp2] (inp3) {\texttt{5}};
\node [left=0.25 of inp2] (inp1) {\texttt{1}};
\path[arrow] (inp2) -- (embed);
\path[arrow] (inp3) -- (embed.south -| inp3);
\path[arrow] (inp1) -- (embed.south -| inp1);
\node [below=0.1 of inp2]{\textbf{Encoder}};
  

\node [box,right=1.0 of embed](emb2){Embedding};

\node [below=0.3 of emb2](enc2){\texttt{3}};
\node [left=0.25 of enc2](enc3){\texttt{BOS}};
\node [below=0.1 of enc2]{\textbf{Decoder}};

\node [box2,above=0.23 of emb2](em22){y$_2$};
\path[draw,thick] (emb2) -- (em22);
\path[arrow] (enc2) -- (emb2);
\path[arrow] (enc3) -- (emb2.south -| enc3);



\node [box2,left=0.25 of em22](em21){y$_1$};
\path[draw,thick] (emb2.north -| em21) -- (em21);

\node [box,above=0.4 of em22,fill=Orange] (selfatt2){Self-attention};
\path[arrow] (em22) -- (selfatt2);
\path[arrow] (em21) -- (selfatt2.south -| em21);

\node [box,above=0.23 of selfatt2] (gate){Copy-gate};
\path[arrow] (selfatt2) -- (gate);

\node [box,above=0.23 of gate,fill=Orange] (XattD){Cross-attention};
\path[arrow] (gate) -- (XattD);

\node [box,above=0.23 of XattD] (ffn) {FCNN};
\path[arrow] (XattD) -- (ffn);

\node [label={[rotate=270]35:Layer 1 (shared)},rectangle,draw,dashed,inner sep=0.7em,fit=(selfatt2) (ffn)] (decoder2) {};
\node [box,above=0.55 of ffn,fill=Orange] (selfatt3){Self-attention};
\path[arrow] (ffn) -- (selfatt3);

\node [box,above=0.23 of selfatt3,fill=Orange] (crossatt2){Cross-attention};
\path[arrow] (selfatt3) -- (crossatt2);

\node [box,above=0.23 of crossatt2] (ffn2) {FCNN};
\path[arrow] (crossatt2) -- (ffn2);
\node [label={[rotate=270]22:Layer 2},rectangle,draw,dashed,inner sep=0.7em,fit=(selfatt3) (ffn2)] (decoder2) {};
\node [box,above=0.4 of ffn2] (linear){Linear classifier};
\path[arrow] (ffn2) -- (linear);
\node [box,above=0.23 of linear] (softmax){Softmax};
\path[arrow] (linear) -- (softmax);
\node[above=0.3 of softmax](output){\texttt{5}};
\path[arrow] (softmax) -- (output);

\coordinate[above right =0.2 and 0.7 of tok3](conn);
\path[draw,thick] (tok1) |- (conn);
\path[draw,thick] (tok2) |- (conn);
\path[draw,thick] (tok3) |- (conn);

\coordinate[left=0.1 of gate](lg);
\path[draw,thick] (gate) -- (lg);
\coordinate[above=0.1 of ffn.north](mw2);
\path[arrow] (lg) |- (mw2);
\coordinate[right=1.5 of mw2](mw3);
\path[draw,thick] (mw2)-- (mw3);
\coordinate[below right =0.1 and 0.1 of selfatt2.south](mw);
\path[arrow] (mw3) |- (mw);
 
\path [arrow] (ffne.north -| tok1) -- (tok1);
\path [arrow] (ffne) -- (tok2);
\path [arrow] (ffne.north -| tok3) -- (tok3);
\path [arrow] (selfatt) -- (ffne);
\path [arrow] (se) -- (selfatt);
\path [arrow] (se2) -- (selfatt.south -| se2);
\path [arrow] (se3) -- (selfatt.south -| se3);
\path[draw,thick] (embed.north -| se2) -- (se2);
\path[draw,thick] (embed) -- (se);
\path[draw,thick] (embed.north -| se3) -- (se3);
\coordinate[left=0.1 of XattD.west](mw4);
\path[arrow] (conn) |- (mw4);
\path[arrow] (conn) |- (crossatt2.west);

\node[draw,text width=3cm] at (-0.2,4.2) {Embedding dimension\\
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt]
\item Encoder: $d_e=1024$ \\
\item Decoder: $d_e=512$ 
\end{itemize}
Attention heads: $4$

Fully connected neural network (FCNN):\\ 
\begin{itemize}[leftmargin=*, itemsep=1pt, topsep=1pt, parsep=1pt]
\item 1 hidden layer \\
\item $4d_e$ neurons \\
\end{itemize}
Shared layer iterated up to $8$ times.
};
\end{tikzpicture}
\caption{\textbf{Our transformer architecture.} }\label{fig:archi}
%\vspace{-0.2cm}
%\end{figure}
\end{minipage}


==> tables/highest_h_256.tex <==
\begin{table}[h]
\small
  \centering
  \vspace{-0.4cm}
    \small\caption{\textbf{Number of nonzero bits in recovered secrets, for n=256.} b = binary, t = ternary, g = Gaussian. 
    }
  \label{tab:highest_h_256}
  \vspace{1mm}
          \resizebox{0.99\textwidth}{!}{%
\begin{tabular}{lccccccccccccccc}
\toprule
$\log_2 q$    &  &  12 & & &  14 & & & 16 & & & 18 & & & 20 & \\ \midrule
secret distribution & b  \hspace{-2mm}     & t  \hspace{-2mm}     & g  \hspace{3mm}     & b  \hspace{-2mm}     & t  \hspace{-2mm}     & g  \hspace{3mm}     & b  \hspace{-2mm}      & t  \hspace{-2mm}     & g  \hspace{3mm}    & b  \hspace{-2mm}      & t  \hspace{-2mm}     & g  \hspace{3mm}    & b  \hspace{-2mm}      & t  \hspace{-2mm}     & g     \\ 
highest $h$   & 8 \hspace{-2mm}       & 9   \hspace{-2mm}     & 6   \hspace{3mm}    & 12  \hspace{-2mm}      & 13    \hspace{-2mm}    & 6    \hspace{3mm}   & 14  \hspace{-2mm}     & 16  \hspace{-2mm}     & 9   \hspace{3mm}   & 23   \hspace{-2mm}     & 23   \hspace{-2mm}    & 9   \hspace{3mm}   & 36    \hspace{-2mm}    & 33   \hspace{-2mm}    & 10  \\ \bottomrule    
\end{tabular}
}
  \vspace{-2mm}
  \end{table}


==> tables/new_model_256.tex <==
\begin{table}[h!]
\small
  \centering
\begin{tabular}{ll|lll|llll}
             & $\log_2 q$          & \multicolumn{3}{c}{12}                               & \multicolumn{4}{c}{14}    \\
             & $h$               & 4          & 5        & 6        & 6    & 7    & 8    & 9    \\
Seq2seq      & full recovery    & 3/10       & 1/10     & 2/10     & 1/10 & 1/10 & 2/10 & 1/10 \\
             & epochs         & 0,5,5      & 7        & 4,7      & 0    & 1    & 1,1  & 1    \\
Encoder-only & full recovery   & 4/10       & 3/10     & 3/10     & 2/10 & 1/10 & 2/10 & 1/10 \\
             & epochs        & 0,15,16,27 & 20,23,27 & 16,23,28 & 1,14 & 1    & 1,2  & 1   
\end{tabular}
\vspace{2mm}
    \small\caption{\textbf{title}. Caption }
    \label{tab:new_model_256}
\end{table}

==> tables/no_mod.tex <==
\begin{table}[t]
\small
  \centering
\resizebox{0.65\textwidth}{!}{
\begin{tabular}{llllllllllll}
$\bf h$ & {\bf method} & \multicolumn{10}{c}{\bf \nomod{} values and recovery success} \\ \midrule
\multirow{2}{*}{$6$}  & orig & 0.56 & 0.61 & 0.60 & 0.61 & 0.56 & 0.52 & 0.67 & 0.67 & \success{0.76} & 0.67  \\
                    & perm & 0.57 & 0.67 & 0.56 & 0.67 & 0.62 & \success{0.67} & 0.60 & 0.60 & \fail{0.52} & 0.56 \\ \midrule
\multirow{2}{*}{$7$}  & orig & 0.60 & 0.60 & 0.52 & 0.49 & 0.60 & \success{0.75} & 0.55 & 0.60 & 0.55 & 0.56  \\
                    & perm & \success{0.67} & 0.52 & 0.60 & \success{0.75} & 0.60 & \success{0.73} & 0.60 & \success{0.71} & 0.59 & 0.66 \\ \midrule
 \multirow{2}{*}{$8$}  & orig & 0.60 & \success{0.74} & \success{0.74} & 0.66 & 0.60 & 0.66 & 0.55 & 0.60 & 0.63 & 0.55  \\ 
                    & perm & 0.55 & 0.55 & 0.60 & 0.52 & 0.55 & 0.60 & 0.55 & 0.49 & 0.60 & 0.60 \\ \bottomrule
\end{tabular}
}
\vspace{2mm}
    \small\caption{\textbf{\nomod{} values and recovery success before/after permuting the columns of $A$}. $n=256, \log_2 q = 14$, binary secrets. $10$ secrets for $3$ values of $h$. \success{Green} $=$ secret recovered; \fail{\em red} or black $=$ failure.}
    \label{tab:permute_cols}
    \vspace{-0.5cm}
\end{table}


==> tables/small_q.tex <==
\begin{table}[h!]
\small
  \centering
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{$n$}   & \multirow{2}{*}{$\log_2 q$} & preproc. time & stddev & \multicolumn{3}{c}{recovered $h$} \\  %\cmidrule{5-7}
                     &                       &                                 (hrs/matrix)   &     ratio                 & b         & t        & g        \\ \midrule
\multirow{5}{*}{256} & 12 & 1.5 & 0.77 & 6  & 6  & 5  \\
                     & 14 & 2.5 & 0.71 & 9  & 9  & 6  \\
                     & 16 & 8.0 & 0.63 & 12 & 12 & 6  \\
                     & 18 & 7.0 & 0.53 & 18 & 19 & 7  \\
                     & 20 & 7.5 & 0.43 & 33 & 25 & 7  \\ \midrule
\multirow{2}{*}{350} & 21 & 16  & 0.61 & 12 & 13 & 5  \\
                     & 27 & 216 & 0.38 & 36 & 38 & 10 \\ \bottomrule
\end{tabular}
\vspace{2mm}
    \small\caption{$n=256$ and $n=350$. Highest $h$ recovered, running on $10$ random secrets for each $h$. Secret distributions are b = binary, t = ternary, g = Gaussian. }
    \label{tab:small_q}
    \vspace{-0.5cm}
\end{table}
